B/PS bulges and barlenses from a kinematic viewpoint. II

Internal dynamics and kinematics of galaxies have imprints on the line-of-sight velocity distribution~(LOSVD). Gauss-Hermite parametrisation allows one to identify the kinematics features of the system in terms of skewness~($h_3$) and broadness~($h_4$) deviations of a LOSVD. Such a method provides information about the type of orbits since a $h_3-\overline V$ correlation is a sign of elongated orbits, and the anti-correlation is a sign of circular or near-circular orbits. In previous works, analysis of the $h_3-\overline V$ relation provided a tool to identify a hidden bar or B/PS bulge~(edge-on, $\mathrm{PA}=90^\circ$) and to probe their strength. We prepared two $N$-body galaxy models with clear B/PS bulges: one has an ordinary bar~(the X model), and the second one has a barlens embedded into a bar~(the BL model) to investigate the mechanism of formation of $h_3$ features at any position of an observer. We show that the $h_3-\overline V$ correlation appears in the regions where bar and disc particles are mixing. We also reveal that the model with a barlens has an $h_3-\overline V$ anti-correlation in the centre, and we show that barlens-specific orbits are responsible for this signal. Moreover, this feature can be observed only for galaxies with compact bulges and barlenses. The results of this work are applicable for the interpretation of future Integral-field unit (IFU) data for real galaxies with B/PS bulges, especially for objects with barlenses.

==> pgfgraphicsmacros.tex <==
\usepackage{adjustbox} 
\usepackage{import} 
% i know what i'm doing!
\makeatletter
\def\import@pgf@picture#1\@end{%
  \def\@dir{}\def\@file{}%
  \parse@paths#1/\relax/%
  \expandafter\expandafter\expandafter\import%
  \expandafter\expandafter\expandafter{\expandafter\@dir\expandafter}\expandafter{\@file}%
} % adapted parser by David Carlisle, https://tex.stackexchange.com/a/84804
\def\parse@paths#1/#2/{%
  \edef\@trailing{#2/}%
  \ifx\relax#2\edef\@file{#1}\edef\@trailing{}%
  \else \edef\@dir{\@dir#1/}\expandafter\expandafter\expandafter\parse@paths\expandafter\fi\@trailing%
}
% \def\@import@pgf@picture#1/#2\@end{\import{#1}{#2}}
\newcommand*{\includepgfgraphics}[2][]{%
  \begingroup%
  \ifx &#1&\import@pgf@picture #2\@end%
  \else \begin{adjustbox}{#1}\import@pgf@picture #2\@end\end{adjustbox}%
  \fi\endgroup%
}
\makeatother


==> tannot/tannot-authors-code.tex <==

% properties
\def \tnt@authors@setup#1{%
  \kv@parse{#1}\tnt@authors@processaliases%
}%

% list-of-names properties
\def \tnt@authors@processaliases#1#2{%
  \def \do##1{\tnt@authors@setupsingle{##1}{#2}}%
  \docsvlist{#1}%
}

% name properties
\def \tnt@authors@setupsingle#1#2{%
  \define@key{tnt@authorprop}{pen color}[tnt@defaults@color]{%
    \definecolor{tnt@authors@#1}{HTML}{##1}%
  }%
  \kv@set@family@handler{tnt@authorprop}{%
    \csgdef{tnt@authors@/#1/##1}{##2}%
  }%
  \kvsetkeys{tnt@authorprop}{#2}%
}

\def \tnt@authors@getprop#1#2{\csuse{tnt@authors@/#1/#2}}

% whom subject ..name
\def \tnt@authors@mailtolink#1#2{
  \ifstrempty{#2}{%
    \href{mailto:\tnt@authors@getprop{#1}{email}}%
  } {%
    \href{mailto:\tnt@authors@getprop{#1}{email}?subject=#2}%
  }%
}

% vim: ft=plaintex


==> tannot/tannot-code.tex <==
% Copyright (c) 2022 Iliya Tikhonenko.
%
% Permission is granted to copy, distribute and/or modify this
% software under the terms of the LaTeX Project Public License
% (LPPL), version 1.3c.
%
% This software is provided 'as is', without warranty of any kind,
% either expressed or implied, including, but not limited to, the
% implied warranties of merchantability and fitness for a
% particular purpose.

% macro guts for tannot.sty

\def\tnt@author@def#1#2{
  \kv@set@family@handler{tnt@authors@#1}{
    \csdef{@tnt@authors@#1@##1}{##2}
  }
}

% vim: ft=plaintex


==> tannot/tannot-commenting-code.tex <==
\def \tnt@boxes@reducedstrut{%
	\vrule width 0pt height .9\ht\strutbox depth .9\dp\strutbox\relax%
}

% #1 = prefix #2 = name
\def \tnt@commenting@setupinlinecommands#1#2{%
	\csdef{#1c}{\tnt@helpers@commenting@capturelabel{\tnt@commenting@highlight{#2}}}%
	\csdef{#1m}{\tnt@helpers@commenting@checkmarkargs{#2}}%
	\csdef{#1ins}{\tnt@helpers@commenting@capturelabel{\tnt@commenting@insert{#2}}}%
	\csdef{#1del}{\tnt@helpers@commenting@capturelabel{\tnt@commenting@delete{#2}}}%
}

\def \tnt@commenting@setupsummarycommands#1#2{%
	\csdef{#1c}{\tnt@commenting@summarycomment{#2}}%
	\csdef{#1m}{\relax}%
	\csdef{#1ins}{\relax}%
	\csdef{#1del}{\relax}%
}

% author = command prefix, ...
\kv@set@family@handler{tnt@commenting@authoroptions}{%
	\edef\@prefix{\ifblank{#2}{#1}{#2}}%
	\tnt@commenting@setupinlinecommands\@prefix{#1}%
}
% author = command prefix, ...
\kv@set@family@handler{tnt@commenting@summaryoptions}{%
	\edef\@prefix{\ifblank{#2}{#1}{#2}}%
	\tnt@commenting@setupsummarycommands{\@prefix}{#1}%
}

% code label-until-{
\def \tnt@helpers@commenting@capturelabel#1#2#{#1{#2}}

% author mark body
\def \tnt@commenting@highlight#1#2#3{%
  \ifmmode \let \mathifmathoutside=\ensuremath \else \let\mathifmathoutside=\relax \fi%
  \colorbox{tnt@authors@#1!15}{%
    \tnt@boxes@reducedstrut%
    \mathifmathoutside{#3}%
    \/%italic correction
  	\ifblank{#2}{}{%
    	\hbox to 0pt{${}^{\textcolor{tnt@authors@#1}{#2}}$}%
  	}%
	}%
}%


\def \tnt@helpers@commenting@checkmarkargs#1#2{%
	\ltx@ifnextchar@nospace[
		{\tnt@helpers@commenting@passmarkargs{#1}{#2}}
		{\tnt@helpers@commenting@passmarkargs{#1}{#2}[]}%
}
\def \tnt@helpers@commenting@passmarkargs#1#2[#3]{\tnt@commenting@mark{#1}{#3}{#2}}

% author mark body 
\def \tnt@commenting@mark#1#2#3{%
  \ifmmode \let \mathifmathoutside=\ensuremath \else \let\mathifmathoutside=\relax \fi%
  %\mbox{%
  	\colorwave{tnt@authors@#1}{\phantom{\mathifmathoutside{#3}}}%
		\llap{\contour{white}{\mathifmathoutside{#3}}}%
	%}%
  \/%italic correction
  \ifblank{#2}{}{%
  	\textsuperscript{[\textcolor{tnt@authors@#1}{\texttt{#2}}]}%
  }%
}%

\def \tnt@commenting@insert#1#2#3{%
  \textcolor{tnt@authors@#1}{#3}%
  \ifblank{#2}{}{%
    \hbox to 0pt{${}^{\textcolor{tnt@authors@#1}{#2}}$}%
  }%
}

\def \tnt@commenting@delete#1#2#3{%
  \ifmmode \let \mathifmathoutside=\ensuremath \else \let\mathifmathoutside=\relax \fi%
  \colorbox{tnt@authors@#1!15}{%
    \tnt@boxes@reducedstrut%
  	\sout{\mathifmathoutside{#3}}%
    % {#3}
    \/%italic correction
  	\ifblank{#2}{}{%
    	\hbox to 0pt{${}^{\textcolor{tnt@authors@#1}{#2}}$}%
  	}%
  }%
}


% author mark body
\def \tnt@commenting@summarycomment#1#2{%
  \ifmmode \let \mathifmathoutside=\ensuremath \else \let\mathifmathoutside=\relax \fi%
  \color{tnt@authors@#1}\hbox{${}^{\text{#2}}$}%
}%

% vim: ft=plaintex


==> tannot/tannot-todo-code.tex <==
\newtoggle{done}
\define@key{tnt@todo}{done}[yes]{%
  \toggletrue{done}%
}


\kv@set@family@handler{tnt@todo}{%
	\let\ex@f=\expandafter%
	\toks@\ex@f\ex@f\ex@f{\ex@f\the\ex@f\toks@\tnt@templates@mention{#1}}%
}

\newwrite\@tnt@todofile
\AtBeginDocument{\immediate\openout\@tnt@todofile=todo.txt}
\AtEndDocument{\immediate\closeout\@tnt@todofile}

% #1=task #2=options (status, whom)
\def \tnt@todo@new#1#2{%
  \begingroup%
	\toks@{}%
	\def\@what{#1}%
  \kvsetkeys{tnt@todo}{#2}%
	\edef\@who{\expandafter\@gobble\the\toks@\relax}%
  \iftoggle{done}
    {\ifdefempty{\@who} \tnt@templates@todo@done \tnt@templates@todo@authordone}
    {\ifdefempty{\@who} \tnt@templates@todo@active \tnt@templates@todo@authoractive}%
  \immediate\write\@tnt@todofile{\iftoggle{done}{x\space}{}\expandonce{\@what} \@who}%
  \endgroup%
}

% vim: ft=plaintex

